It's All Relative! -- A Synthetic Query Generation Approach for Improving Zero-Shot Relevance Prediction

Recent developments in large language models (LLMs) have shown promise in their ability to generate synthetic query-document pairs by prompting with as few as 8 demonstrations. This has enabled building better IR models, especially for tasks with no training data readily available. Typically, such synthetic query generation (QGen) approaches condition on an input context (e.g. a text document) and generate a query relevant to that context, or condition the QGen model additionally on the relevance label (e.g. relevant vs irrelevant) to generate queries across relevance buckets. However, we find that such QGen approaches are sub-optimal as they require the model to reason about the desired label and the input from a handful of examples. In this work, we propose to reduce this burden of LLMs by generating queries simultaneously for different labels. We hypothesize that instead of asking the model to generate, say, an irrelevant query given an input context, asking the model to generate an irrelevant query relative to a relevant query is a much simpler task setup for the model to reason about. Extensive experimentation across seven IR datasets shows that synthetic queries generated in such a fashion translates to a better downstream performance, suggesting that the generated queries are indeed of higher quality.

==> images/prompts.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Prompt-Based QGen Model} & &   \\
\midrule
Generate-Relevant-Only & inputs: & product: {\texttt{passage}}  \\
\cite{dai2022promptagator} & outputs: & query: {\texttt{relevant query}} \\
\midrule
Label-Conditioned & inputs: & product: {\texttt{passage}} label: \texttt{relevant/irrelevant} \\
 \cite{chaudhary2023exploring} & outputs: & query: \texttt{relevant/irrelevant query} \\
\midrule
Pairwise & inputs: & product: {\texttt{passage}} \\
 (Proposed)        & outputs: & query1: {\texttt{relevant query}} \\
 & & query2: {\texttt{irrelevant query}} \\


\bottomrule
\end{tabular}
}
\caption{Comparing prompts across different QGen models.
}
\label{tab:prompt_formats_}
\end{table*}

==> proposedwork.tex <==


\section{Proposed Work: Pairwise Query Generation} \label{ref:proposed}
The above-described QGen approaches, both the label-conditioned \cite{chaudhary2023exploring} and the non-label conditioned Promptagator \cite{dai2022promptagator}, generate queries in isolation of other queries.
As motivated in the introduction, humans find comparing two outputs with respect to each other easier as opposed to evaluating an output in isolation \cite{christiano2017deep}
This makes us wonder whether formulating the QGen task in a similar fashion would lead to high-quality synthetic data.
Below we describe our proposed QGen model in more detail, following the same three steps as presented above:

\paragraph{Generate Query}
Our main innovation lies in this first step of query generation.
Specifically, we propose pairwise query generation, where given an input document, the model is required to generate both the relevant and the irrelevant query.
Like before, we  construct an instruction prompt $p$ using $k$ input-output examples, where the input is a document $d$ and and the output is a pair of queries $(q_{\text{rel}}, q_{\text{irrel}})$ where the first query $q_{\text{rel}}$ is relevant to the $d$ while the second query $q_{\text{irrel}}$ is irrelevant.
The pairwise prompt, therefore, is as follows:
$p\!=\!\{(d_i, q_\text{rel}, q_\text{irrel})^k, d_t\}$.
Given a new document, the model is expected to generate both the relevant and the irrelevant queries at the same time, as shown in \autoref{tab:prompt_formats}.
By forcing the model to generate both queries, the generation of the irrelevant query is conditioned on the previously generated relevant query along with the input context.

\paragraph{Filter Query}
Next, we apply the round-trip consistency filter to remove noisy queries.
We prompt the LLM again, but this time to predict whether the generated synthetic query $q_{\text{syn}}$ is relevant or not to the document $d_t$ from which it was generated.
Specifically, the prompt comprises of $k$ query-document example pairs across both relevance labels:
$p_{\text{filter}}\!=\!\{(q_i, d_i, l_i)^k, (q_{\text{syn}}, d_t)\}$, where $l \in L\!=\!\{\text{relevant}, \text{irrelevant}\}$.
We apply the $p_{\text{filter}}$ on the synthetic query-document pair $(q_{\text{syn}}, d_t)$ and compute the log-likelihood to score each output label $L$, given the prompt.
Then, we select the label with the highest score, as shown below:
$l_{\text{pred}} = \argmax_{L} \text{score}(l, p_{\text{filter}})$ where $p$ refers to the filtration prompt and \emph{score} is the log-likelihood.
As described in \autoref{ref:filter}, we only retain those queries whose predicted label $l_{\text{pred}}$ matches the label for which the query was generated.
For instance, in our proposed pairwise QGen, the first query will be retained only if it is rated as relevant and, similarly, the second query if it is rated as not relevant.
In addition to the round-trip filtering, we also remove duplicate queries i.e. queries that got labeled with different relevance labels for the same document, following \citet{chaudhary2023exploring}.

\paragraph{Train Downstream Model}
Finally, using the above generated and filtered synthetic query-document, we train a relevance prediction model for each of the target tasks.
Note that through our proposed method, the model is able to generate training examples for both relevant and irrelevant labels, alleviating the need of running the additional step of an retriever \cite{dai2022promptagator}.
In the next section, we describe our experimental setup.
